Saturated Overburden Scattering and the Multiscatter Frontier: Discovering Dark Matter at the Planck Mass and Beyond

We show that underground experiments like LUX/LZ, PandaX-II, XENON, and PICO could discover dark matter up to the Planck mass and beyond, with new searches for dark matter that scatters multiple times in these detectors. This opens up significant discovery potential via re-analysis of existing and future data. We also identify a new effect which substantially enhances experimental sensitivity to large dark matter scattering cross-sections: while passing through atmospheric or solid overburden, there is a maximum number of scatters that dark matter undergoes, determined by the total number of scattering sites it passes, such as nuclei and electrons. This extends the reach of some published limits and future analyses to arbitrarily large dark matter scattering cross-sections.

==> universalnewcommands.tex <==
\newcommand{\half}{\frac{1}{2}}
\newcommand{\gsim}{\gtrsim}
\newcommand{\lsim}{\lesssim}
\newcommand{\ra}{\rightarrow}
\newcommand{\mtop}{m_t}
\newcommand{\ct}{c_\theta}
\newcommand{\st}{s_\theta}
\def\sigmaveeave{\langle \sigma v\rangle}
\def\sigmaveeann{\langle \sigma v\rangle_{\rm ann}}
\def\relabund{\Omega_\chi h^2}
\def\lag{\mathcal{L}}
\def\Oc{\mathcal{O}}
\def\Mc{\mathcal{M}}
\def\shat{\sqrt{\hat{s}}}
\def\shatsq{\sqrt{s}}
\def\met{\slashed{E}_T}


\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}
